Fairness in Token Delegation: Mitigating Voting Power Concentration in DAOs

Decentralized Autonomous Organizations (DAOs) aim to enable participatory governance, but in practice face challenges of voter apathy, concentration of voting power, and misaligned delegation. Existing delegation mechanisms often reinforce visibility biases, where a small set of highly ranked delegates accumulate disproportionate influence regardless of their alignment with the broader community. In this paper, we conduct an empirical study of delegation in DAO governance off-chain discussions from 14 DAO forums. We develop a methodology to link forum participants to on-chain addresses, extract governance interests using large language models, and compare these interests against delegates' historical behavior. Our analysis reveals that delegations are frequently misaligned with token holders' expressed priorities and that current ranking-based interfaces exacerbate power concentration. We argue that incorporating interest alignment into delegation processes could mitigate these imbalances and improve the representativeness of DAO decision-making. To support future research, we will release our dataset and code in a public repository.

==> preamble.tex <==
%! TEX root = ../main.tex
% \RequirePackage{amsmath}
% \documentclass[runningheads]{llncs}
% \let\proof\relax\let\endproof\relax % To use amsthm together with llncs

% \documentclass{article}
% \usepackage[letterpaper]{geometry}
% \pagenumbering{gobble}
% \input{preamble}
% \begin{document}
% \author{
% Aviv Yaish$^{1,3}$ \and
% Benjamin Livshits$^{2,3}$
% }
% \date{
% $^1$The Hebrew University of Jerusalem, Israel \\
% $^2$Imperial College London, UK \\
% $^3$Matter Labs
% }

%% Ifs
\newif\iflong   % For longer versions of the paper
\newif\ifmorecites
\newif\ifanonymous
\newif\ifcomments   % For our comments

\anonymousfalse
\commentstrue
% \anonymoustrue
% \commentsfalse

% %% Try to reduce the number of lines
% \everypar{\looseness=-1 }   % Can be reduced (need a space to terminate the number, otherwise if the paragraph started with 3 \looseness would be set to -13)
% \linepenalty=8000           % Can be increased
% \raggedbottom               % This can be used if we don't want text to fill the entire vertical space of the page, and this can also save space in the beginning of the document

%% Packages
\usepackage[T1]{fontenc}    % Forces T1 fonts, which are supposed to be nicer than the standard ones
\usepackage[english]{babel} % Allows to use special characters, translates some elements within the document, automatically activates the appropriate hyphenation rules for the language you choose. 
\usepackage{mathtools}      % For creating paired delimiters, such as ceil
% \usepackage[english]{babel} % Allows to use special characters, translates some elements within the document, automatically activates the appropriate hyphenation rules for the language you choose. 
% \usepackage{subcaption}     % Allows putting figures side-by-side or one-on-top-of-the-other
% \usepackage[ruled,linesnumbered]{algorithm2e} % For algorithms
\usepackage{enumitem}       % For creating nice enumerated environments
\usepackage{graphicx}       % For specifying image location
\graphicspath{ {./images/} }
\usepackage{booktabs}       % Pretty tables
\usepackage{array,multirow} % For multiple rows/columns in tables
\usepackage{tabularx}       % Can specify column length in tables
% \usepackage{amsthm}         % To manually create theorem environments
\usepackage{amsfonts}
\usepackage{thmtools,thm-restate}   % To restate theorems (define them in one place, and then restate them someplace else)
\usepackage{xcolor}         % Can set nice colors for hyperlinks
\usepackage{hyperref} % For linking to websites
\hypersetup{                % Remove boxes from links, color them instead
    colorlinks,
    linkcolor={red!50!black},
    citecolor={blue!50!black},
    urlcolor={blue!80!black}
}
% \usepackage{minted} % For embedding code, e.g. python
% \usemintedstyle{colorful} % See available styles here https://www.overleaf.com/learn/latex/Code_Highlighting_with_minted#Reference_guide
\usepackage{csquotes}       % Nicer quotes, uses special commands, see https://tex.stackexchange.com/a/39302
\usepackage[capitalise]{cleveref}       % Automatically adds "Section", "Table", etc' to references. Should be imported after all packages
% \usepackage{subfiles} % For working with multiple content .tex files, allows each file to be compiled separately, best loaded last in the preamble

%% Comments
\setlength {\marginparwidth }{2cm}  % Increase margins for notes
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny,textwidth=\marginparwidth]{todonotes}
\newcommand{\aviv}[1]{\ifcomments {\todo[color=blue!40,inline]{Aviv: #1}} \fi}
\newcommand{\ben}[1]{\ifcomments {\todo[color=red!40,inline]{Ben: #1}} \fi}

%% Theorems
% \newtheorem{definition}{Definition}
% \newtheorem{theorem}{Theorem}
% \newtheorem{claim}{Claim}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \newtheorem{example}{Example}
% \newtheorem*{example*}{Example}
% \newtheorem{casestudy}{Case Study}
% \newtheorem*{casestudy*}{Case Study}
% \newtheorem*{discussion*}{Discussion}
% \newtheorem{remark}{Remark}

%% Define reference labels, for cleveref
\crefname{definition}{Definition}{Definitions}
\crefname{theorem}{Theorem}{Theorems}
\crefname{claim}{Claim}{Claims}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{example}{Example}{Examples}
\crefname{remark}{Remark}{Remarks}
\crefname{code}{Code}{Code}

%% Math operators
\DeclareMathOperator*{\argmax}{arg\,\max}
\DeclareMathOperator*{\argmin}{arg\,\min}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\newcommand{\expectation}[1]{\mathrm{E} \left[ {#1} \right]}
\newcommand{\variance}[1]{\mathrm{Var} \left[ {#1} \right]}
\newcommand{\define}{\stackrel{\mathclap{\tiny\mbox{def}}}{=}}

%% Glossary (Acronyms and Notations)
% For easily creating a table of glossaries and acronyms. "glossaries-extra" has nice built-in support for symbols, while "glossaries" doesn't
% If entries are not sorted, nogroupskip prevents adding random whitespace between them
% Using '\gls[hyper=true]{bitcoin}' will cancel the automatic hyperlink
\usepackage[symbols,acronym,nonumberlist,nogroupskip,stylemods={mcols,longbooktabs},section=subsection]{glossaries-extra}
% \makenoidxglossaries

% Acronyms
\setabbreviationstyle[acronym]{long-short}  % Will show the first acronym like so: <long-version> (<short-version>)
\glssetcategoryattribute{acronym}{nohyper}{true} % Disable 

\newacronym[longplural={Markov decision processes}]{MDP}{MDP}{Markov decision process}
\newacronym{AI}{AI}{artificial intelligence}
\newacronym{AMM}{AMM}{automated market maker}
\newacronym{APY}{APY}{annual percentage yield}
\newacronym{APR}{APR}{per block interest rate (non compounding)}
\newacronym{ASIC}{ASIC}{application specific integrated circuit}
\newacronym{CDF}{CDF}{cumulative density function}
\newacronym{CPU}{CPU}{central processing unit}
\newacronym{DAA}{DAA}{difficulty-adjustment algorithm}
\newacronym{DQL}{DQL}{deep-Q-learning}
\newacronym{DeFi}{DeFi}{decentralized finance}
\newacronym{EIP}{EIP}{Ethereum improvement proposal}
\newacronym{ERC}{ERC}{Ethereum request for comments}
\newacronym{EVM}{EVM}{Ethereum virtual machine}
\newacronym{HUJI}{HUJI}{Hebrew University of Jerusalem, Israel}
\newacronym{LP}{LP}{liquidity provider}
\newacronym{LT}{LT}{liquidity taker}
\newacronym{MEV}{MEV}{miner-extractable value}
\newacronym{BEV}{BEV}{blockchain-extractable value}
\newacronym{ML}{ML}{machine learning}
\newacronym{OO}{OO}{order optimization}
\newacronym{PDF}{PDF}{probability density function}
\newacronym{PID}{PID}{proportional integral derivative}
\newacronym{PoS}{PoS}{proof-of-stake}
\newacronym{PoW}{PoW}{proof-of-work}
\newacronym{RAM}{RAM}{random-access memory}
\newacronym{RL}{RL}{reinforcement learning}
\newacronym{RPC}{RPC}{remote procedure call}
\newacronym{SSD}{SSD}{solid state drive}
\newacronym{TD}{TD}{total difficulty}
\newacronym{URL}{URL}{uniform resource locator}
\newacronym{USD}{USD}{United States Dollar}
\newacronym{WETH}{WETH}{Wrapped Ethereum}
\newacronym{WBTC}{WBTC}{Wrapped Bitcoin}
\newacronym{YAML}{YAML}{YAML Ain't Markup Language}
\newacronym{block-DAG}{block-DAG}{block directed-acyclic-graph}
\newacronym{geth}{geth}{Go Ethereum}
\newacronym{p2p}{p2p}{peer to peer}
\newacronym{FaaS}{FaaS}{front-running-as-a-service}
\newacronym{FSL}{FSL}{fixed spread liquidation}
\newacronym{DEX}{DEX}{decentralized exchange}
\newacronym{TVL}{TVL}{total value locked}
\newacronym{CPAMM}{CPAMM}{constant product automated market maker}
\newacronym{CFMM}{CFMM}{constant function market maker}
\newacronym{TFM}{TFM}{transaction fee mechanism}
\newacronym{IC}{IC}{incentive compatible}
\newacronym{FN}{FN}{false name}
\newacronym{MIC}{MIC}{miner incentive compatible}
\newacronym{wrt}{w.r.t.}{with regards to}
\newacronym{QoS}{QoS}{Quality-of-Service}
\newacronym{NFT}{NFT}{non-fungible token}
\newacronym{ENS}{ENS}{Ethereum Name Service}
\newacronym{L1}{L1}{layer-1 blockchain}
\newacronym{L2}{L2}{layer-2 blockchain}


%% Paper notations
\glsxtrnewsymbol[description={
    A single block.
}]{block}{
    \ensuremath{b}
}
\newcommand{\block}{{\gls[hyper=false]{block}}}

\setcounter{topnumber}{4}
\setcounter{bottomnumber}{4}
\setcounter{totalnumber}{8}


